A very deep Chandra observation of Abell 1795: The Cold Front and Cooling Wake

We present a new analysis of very deep Chandra observations of the galaxy cluster Abell 1795. Utilizing nearly 750 ks of net ACIS imaging, we are able to resolve the thermodynamic structure of the Intracluster Medium (ICM) on length scales of ~ 1 kpc near the cool core. We find several previously unresolved structures, including a high pressure feature to the north of the BCG that appears to arise from the bulk motion of Abell 1795's cool core. To the south of the cool core, we find low temperature (~ 3 keV), diffuse ICM gas extending for distances of ~ 50 kpc spatially coincident with previously identified filaments of H-alpha emission. Gas at similar temperatures is also detected in adjacent regions without any H-alpha emission. The X-ray gas coincident with the H-alpha filament has been measured to be cooling spectroscopically at a rate of ~ 1 Solar Masses/ yr, consistent with measurements of the star formation rate in this region as inferred from UV observations, suggesting that the star formation in this filament as inferred by its H$\alpha$ and UV emission can trace its origin to the rapid cooling of dense, X-ray emitting gas. The H-alpha filament is not a unique site of cooler ICM, however, as ICM at similar temperatures and even higher metallicities not cospatial with H$\alpha$ emission is observed just to the west of the H-alpha filament, suggesting that it may have been uplifted by Abell 1795's central active galaxy. Further simulations of cool core sloshing and AGN feedback operating in concert with one another will be necessary to understand how such a dynamic cool core region may have originated and why the H-alpha emission is so localized with respect to the cool X-ray gas despite the evidence for a catastrophic cooling flow.

==> Table.tex <==
493  &  2000-03-21  &  207.3594  &  26.7648  &  19.38  \\
494  &  1999-12-20  &  207.1612  &  26.6324  &  17.47  \\
3666  &  2002-06-10  &  207.2991  &  26.5763  &  12.65  \\
5286  &  2004-01-14  &  207.2740  &  26.6759  &  14.29  \\
5287  &  2004-01-14  &  207.1615  &  26.6319  &  14.30  \\
5288  &  2004-01-16  &  207.1064  &  26.6186  &  14.49  \\
5289  &  2004-01-18  &  206.9230  &  26.6856  &  14.95  \\
5290  &  2004-01-23  &  207.0570  &  26.7557  &  14.95  \\
6159  &  2005-03-20  &  207.0488  &  26.4892  &  14.85  \\
6160  &  2005-03-20  &  207.1989  &  26.5243  &  14.84  \\
6161  &  2005-03-28  &  207.3613  &  26.4856  &  13.59  \\
6162  &  2005-03-28  &  207.2836  &  26.5707  &  13.60  \\
6163  &  2005-03-31  &  207.2787  &  26.5541  &  14.85  \\
10432  &  2009-03-16  &  207.4147  &  26.3368  &  5.10  \\
10898  &  2009-04-20  &  207.3060  &  26.5316  &  15.73  \\
10899  &  2009-04-22  &  207.2275  &  26.6171  &  14.92  \\
10900  &  2009-04-20  &  207.2440  &  26.5468  &  15.82  \\
10901  &  2009-04-20  &  207.2756  &  26.3634  &  15.47  \\
12026  &  2010-05-11  &  207.2914  &  26.5987  &  14.92  \\
12027  &  2010-03-16  &  207.2363  &  26.5942  &  14.85  \\
12028  &  2010-05-10  &  207.2445  &  26.5371  &  14.97  \\
12029  &  2010-04-28  &  207.2395  &  26.5838  &  14.33  \\
13106  &  2011-04-01  &  207.2666  &  26.4899  &  9.91  \\
13107  &  2011-04-01  &  207.2034  &  26.5869  &  9.64  \\
13108  &  2011-03-10  &  207.2628  &  26.4877  &  14.86  \\
13109  &  2011-03-11  &  207.2369  &  26.5795  &  14.58  \\
13110  &  2011-03-11  &  207.2666  &  26.5242  &  14.58  \\
13111  &  2011-03-11  &  207.1874  &  26.5652  &  14.58  \\
13112  &  2011-03-11  &  207.2661  &  26.5388  &  14.58  \\
13113  &  2011-03-11  &  207.2110  &  26.5535  &  14.58  \\
13412  &  2011-05-22  &  207.4045  &  26.7287  &  14.86  \\
13413  &  2011-05-29  &  207.3675  &  26.7338  &  14.85  \\
13414  &  2011-05-29  &  207.4582  &  26.5656  &  14.57  \\
13415  &  2011-05-29  &  207.4892  &  26.5774  &  14.58  \\
13416  &  2011-05-30  &  207.3197  &  26.5420  &  14.58  \\
13417  &  2011-06-02  &  207.1801  &  26.3135  &  14.86  \\
14268  &  2012-03-26  &  206.9323  &  26.7224  &  9.93  \\
14269  &  2012-04-08  &  207.2240  &  26.5826  &  9.94  \\
14270  &  2012-03-25  &  207.2699  &  26.4912  &  14.28  \\
14271  &  2012-03-25  &  207.0160  &  26.7243  &  13.98  \\
14272  &  2012-03-25  &  207.2802  &  26.6434  &  14.58  \\
14273  &  2012-03-26  &  207.3302  &  26.3056  &  14.58  \\
14274  &  2012-04-02  &  207.2381  &  26.5873  &  14.88  \\
14275  &  2012-04-07  &  207.4440  &  26.5319  &  14.88  \\
15485  &  2013-04-21  &  207.2652  &  26.5321  &  9.94  \\
15486  &  2013-04-22  &  207.2284  &  26.5816  &  9.65  \\
15487  &  2013-06-02  &  207.2980  &  26.6725  &  14.63  \\
15488  &  2013-04-10  &  207.2653  &  26.5709  &  14.58  \\
15489  &  2013-04-08  &  207.2637  &  26.6476  &  14.58  \\
15490  &  2013-04-17  &  207.4697  &  26.4087  &  14.89  \\
15491  &  2013-04-18  &  207.2150  &  26.4544  &  14.89  \\
15492  &  2013-04-15  &  207.5037  &  26.6057  &  14.58  \\
